Dynamically Reconfigurable Photon Exchange in a Superconducting Quantum Processor

Realizing the advantages of quantum computation requires access to the full Hilbert space of states of many quantum bits (qubits). Thus, large-scale quantum computation faces the challenge of efficiently generating entanglement between many qubits. In systems with a limited number of direct connections between qubits, entanglement between non-nearest neighbor qubits is generated by a series of nearest neighbor gates, which exponentially suppresses the resulting fidelity. Here we propose and demonstrate a novel, on-chip photon exchange network. This photonic network is embedded in a superconducting quantum processor (QPU) to implement an arbitrarily reconfigurable qubit connectivity graph. We show long-range qubit-qubit interactions between qubits with a maximum spatial separation of $9.2~\text{cm}$ along a meandered bus resonator and achieve photon exchange rates up to $g_{\text{qq}} = 2\pi \times 0.9~\text{MHz}$. These experimental demonstrations provide a foundation to realize highly connected, reconfigurable quantum photonic networks and opens a new path towards modular quantum computing.

==> QQCoupling_old.tex <==
The effective qubit-qubit coupling Hamiltonian mediated by the Bus can be obtained through time-dependent Schrieffer-Wolff transformation (tSWT) using the following transformation $S_1$ (see Appendix.~\ref{} for details) with $a$($a^{\dagger}$) and $\sigma_{i,-}$($\sigma_{i,+}$) as the annialation(creation) operators for a photon in Bus and qubit-$i$ respectively.
\begin{equation}
    S_{1}=\sum_{i=1,2}\left(c_{i}a^{\dagger}\sigma_{i,-}-c_{i}^{*}a\sigma_{i,+}+d_{i}a^{\dagger}\sigma_{i,+}-d_{i}^{*}a\sigma_{i,-}\right)
\end{equation}
where the coefficients $c_{i}$ and $d_{i}$ have the following form:
\begin{align}
    \label{eq:ci}
    c_{i}(t)&=\frac{g_{0i}}{(\Delta_{i}-\omega)(\Delta_{i}+\omega)}\big[\Delta_{i}\cos(\omega t+\phi) \notag \\
    &\ \ \ \ \ -i\omega \sin(\omega t+\phi)-e^{-i\Delta_{i}t}\left(\Delta_{i}\cos\phi -i\omega\sin\phi\right)\big] \\
    \label{eq:di}
    d_{i}(t)&=\frac{g_{0i}}{(\Sigma_{i}-\omega)(\Sigma_{i}+\omega)}\big[-\Sigma_{i}\cos(\omega t+\phi) \notag \\
    &\ \ \ \ \ +i\omega \sin(\omega t+\phi)+e^{-i\Sigma_{i}t}\left(\Sigma_{i}\cos\phi-i\omega\sin\phi\right)\big].
\end{align}
This is straightforward to compute, and in terms of the $c_{i}$ and $d_{i}$ the transformed Hamiltonian becomes, through second order effective Hamiltonian $H_{\text{eff}}^{(2)}=-\frac{1}{2}[S_{1},H_{1}]+H_{2}$ and setting $g_{12}=0$,
\small
\begin{align}
    H'&=a^{\dagger}a\Big[\omega_{\text{r}}+\underbrace{\frac{1}{2}\sum_{i=1,2}g_{i}(t)\sigma_{i,z}(c_{i}+c_{i}^{*}+d_{i}+d_{i}^{*})}_{\text{AC Stark Shift}}\Big] \notag \\
    &\ \ \ +\sum_{i=1,2}\frac{1}{2}\sigma_{i,z}\Big[\omega_{i}+\underbrace{\frac{3}{2}g_{i}(t)(c_{i}+d_{i}+c_{i}^{*}+d_{i}^{*})}_{\text{Lamb Shift}}\Big] \notag \\
    &\ \ \ -\underbrace{\frac{1}{4}\sum_{i=1,2}g_{i}(t)(-c_{i}-c_{i}^{*}+d_{i}+d_{i}^{*})}_{\text{overall energy shift}} \notag \\\
    &\ \ \ -\underbrace{\frac{1}{2}\left(a^{\dagger}\right)^{2}\sum_{i=1,2}\left[g_{i}(t)\sigma_{i,z}(c_{i}+d_{i})+\text{h.c.}\right]}_{\text{state dependent squeezing}} \notag \\
    &\ \ \ -\underbrace{\sigma_{1,-}\sigma_{2,+}\frac{1}{2}\left[g_{1}(t)(d_{2}-c_{2}^{*})+g_{2}(t)(-c_{1}+d_{1}^{*})\right]+\text{h.c.}}_{\text{photon exchange interaction}} \notag \\
    &\ \ \ -\underbrace{\sigma_{1,+}\sigma_{2,+}\frac{1}{2}\left[g_{1}(t)(c_{2}^{*}-d_{2})+g_{2}(t)(c_{1}^{*}-d_{1})\right]+\text{h.c.}}_{\text{two photon creation/annihilation interaction}}
\end{align}
\normalsize
Next we insert the expressions for $c_{i}(t)$ and $d_{i}(t)$ from Eqns.~\ref{eq:ci} $-$ \ref{eq:di} with $\omega=\tilde{\Delta}_{12}/2$. Lastly, Eqn.~\ref{eq:Hinteff} is recovered by moving to the interaction picture and making the rotating wave approximation, keeping only the static terms in the interacting frame (as outlined in Sec.~\ref{sec:ReconQPU}).
\todo{need to put a simplified hamiltonian here}

We observed desired parametric coherent photon exchanged between qubit pairs (see Fig.~\ref{} for Qubit-1 and Qubit-4). By repeating the time-domain experiment between Qubit-1 and Qubit-4 for different Bus flux modulation amplitudes, we extract the photon exchange rate as a function of Bus modulating amplitude shown in Fig.~\ref{} as red dots. We also overlay the theory prediction (dashed line) based on independently measured system parameters from previous data fit of qubit-bus coupling. The close alignment between theory prediction and independent experimental observation highlights the accuracy of dynamics model developed in this work used to guide the implementation of this work's physical device.

Similar pairwise coherent photon exchange experiments are carried between 5 operational qubits and we identified 8 pairwise parametric photon exchange routes enabled on-demand by respective Bus flux modulation frequencies (see Appendix~\ref{}). It should be noted that a long distance coherent photon exchange was observed between Qubit-1 and Qubit-8 separated by $\sim 9.2~\text{cm}$ along the meandered CPW of the BUS. The direct photon exchange between qubits mediated by almost $10~\text{cm}$ CPW demonstrates the possibility of applying this architecture to entangling qubits on different standard $1~\text{cm}\cross 1~\text{cm}$ quantum chips. In the following section, we calibrated the qubit-qubit gate and characterized its fidelity.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> modulatedBus.tex <==
\begin{figure*}
    \centering
    \includegraphics{figure/parametricQubitBus_horizontal2.pdf}
    \caption{\textbf{a}, Measured (dots) and theory predicted (solid lines) parametric Q$_{4}$-Bus coupling as a function of Bus flux modulation frequency at various modulation amplitudes. The inset of \textbf{a} shows the full 2D theory prediction for $\bar{g}_{4}$ over the relevant parameter ranges with system parameters extracted from fitting the experimental data (see discussion in SI Note~\ref{sec:busmatrixtheory} for details). The dashed white lines in the inset indicate constant modulation amplitude linecuts corresponding to the solid lines in \textbf{a}. \textbf{b}, A typical parametric avoided crossing between Q$_{4}$ and Bus from which the parametric coupling data in \textbf{a} was extracted. \textbf{c}, Parametric couplings between different qubits and the Bus at fixed amplitude ($\delta f=0.104\pi$) and various detunings are extracted from fitting avoided crossings like \textbf{b} and demonstrate that all qubits are coupled symmetrically to the shared Bus as expected. \textbf{d}, Q$_{1}$-Bus parametric coupling rate (red dots) obtained from the photon exchange rate in time domain (TD) and overlaid on the previously obtained parametric coupling rate (blue diamond) from fitting frequency domain (FD) avoided crossings. \textbf{e}, The pulse sequence for measuring time domain coupling rates in \textbf{c}. \textbf{f}, The parametric photon transition process between Q$_{1}$ and Bus at rate $g_{\text{par},1}$ activated by the flux drive to Bus boundaries.}%\textbf{c}, Q$_{1}$-Bus parametric photon exchange using the pulse sequence in \textbf{d}. } %(left) and qubit-Bus transition level diagram (right) for extracting parametric couplings from time-domain photon exchange rates between qubits and Bus.%
    \label{fig:parametricqubitbus}
\end{figure*}
In order to generate parametric photon exchange between qubits, we need to apply a time dependent external flux to the Bus boundary SQUIDs. This modulation of the Bus boundary condition modulates the Bus mode profile and produces a time-periodic coupling between the qubits and Bus. To show this more explicitly, we now investigate the response of the resonance mode field profile under periodic boundary flux modulation, $f_{\pm}(t)=F_{\pm} + \delta f_{\pm} \cos(\omega_{\mathrm{f}}t+\psi_{\pm})$. For simplicity, we assume the static bias points of the two SQUIDs are the same, $F=F_{+}=F_{-}$ as well as their modulation amplitudes, $\delta f=\delta f_{+}=\delta f_{-}$. We Fourier transform and linearize the equations of motion, Eqn.~\ref{eqn:eombndry}, and then decompose the Fourier amplitudes into left and right travelling wave components, $\phi_{\pm}(\omega)$. After taking advantage of the system symmetries (details in SI Note~\ref{sec:busmatrixtheory}), we arrive at an infinite dimensional matrix equation for the vector of sideband phase field amplitudes, $\phi_{\pm}(\omega_{p})$,
\begin{equation}
    \label{eq:matrixformBus}
    \left(\mathbf{\Sigma}\pm\mathbf{\Sigma}^{*}\right)\tilde{\mathbf{\Phi}}_{\pm}=0
\end{equation}
where $\mathbf{\Sigma} = \mathbf{\Lambda}(\{e^{-i\frac{1}{2} \pi n}\})\mathbf{M_{+,+}}\mathbf{\Lambda}(\{e^{i\frac{1}{2} \pi n}\})$ is defined in terms of the matrix 
\begin{multline}\label{eq:freqmatrixelementmain}
     [\mathbf{M}_{s=\pm,z=\pm}]_{mp}=\big[(-\alpha\omega_p^2+sz\eta \ell k_p i)\delta_{mp}+\\
     (e^{iF}+(-1)^{m-p}e^{-iF})J_{p-m}(\delta f)e^{z i\frac{\psi_0}{2}(p-m)}\big]e^{sz\frac{\omega_p \ell}{2v}i}
\end{multline}
and $\mathbf{\Lambda}(\{x_{n}\})$ is the diagonal matrix with $n$th diagonal element $x_{n}$. Additionally, $\delta_{mp}$ is the Kronecker-$\delta$ symbol, $\alpha=2/\omega_{\mathrm{J}}^{2}$, $\psi_{0}=\psi_{+}-\psi_{-}$ is the relative phase between the periodic modulation at either boundary, $J_{p-m}$ is the $(p-m)$th Bessel function of the first kind, and $\omega_{p}=vk_{p}=\omega_{\mathrm{r}} + p\omega_{\mathrm{f}}$ is the $p$th sideband frequency with respect to the tunable Bus resonance frequency $\omega_{\mathrm{r}}$. The symmetric($+$)/anti-symmetric($-$) frequency component vector $\tilde{\mathbf{\Phi}}_{\pm}$ is defined such that $\tilde{\mathbf{\Phi}}_{\pm} = \mathbf{\Lambda}(\{e^{-i\frac{1}{2} \pi n}\})(\mathbf{\Phi}_{+} \pm \mathbf{\Phi}_{-})/\sqrt{2}$ where $\mathbf{\Phi}_{\pm} = (\dots,\tilde{\phi}_{\pm}(\omega_{-1}),\tilde{\phi}_{\pm}(\omega_{0}),\tilde{\phi}_{\pm}(\omega_{1}),\dots)$ is a vector of right($+$)/left($-$) propagating wave frequency components. Parametric boundary flux modulation leads to mixing between different sidebands spaced by $\omega_{\text{f}}$ such that the new normal modes of the system are linear combinations of various sidebands.

% As discussed in Appendix~\ref{sec:busmatrixtheory}, under most conditions the different modes of the Bus do not interact and Eqn.~\ref{eq:matrixformBus} is a valid description of the sideband amplitude behavior of the $n$th order Bus mode when we set $\omega_{\text{r}}=\omega_{n,\text{r}}$. Since the Bus has spatial inversion symmetry the modes are even ($+$) or odd ($-$) under spatial inversion, $\mathbf{\Phi}_{+}=\pm\mathbf{\Phi}_{-}$. For odd (even) modes we solve Eqn.~\ref{eq:matrixformBus} for the case of the minus (plus) sign. At $F=0$ ($F=\pi/2$) corresponding to shorted (open) boundary conditions, the $n$th order mode is even when $n$ is odd (even) and odd when $n$ is even (odd). 
% Spatial symmetry of the modes transitions as a function of boundary bias when $Z(F) \approx Z_{0}$. For the measurements below we fix the operating point at $F=\pi/4$ and the modes have the same spatial symmetry as they do at $F=0$ since $Z(\pi/4) < Z_{0}$. Thus, since we are interested in the behavior of the 8th order mode which dominantly mediates the coupling, we solve $(\Sigma - \Sigma^{*})\tilde{\mathbf{\Phi}}_{-}=0$ from this point on.

We solve numerically for the device parameters in Table~\ref{tab:DCfitpars}, obtained from fitting the Bus spectrum to the circuit model (except symmetric SQUIDs, $d=0$, are assumed) after truncating Eqn.~\ref{eq:matrixformBus} to the $D=3$ lowest sidebands. We compute the coupling strength between the Bus and the qubits with the modulation frequency, $\omega_{\mathrm{f}} = \Delta_{i}$ for qubit $i$ (Q$_i$), generating a resonant parametric interaction between the qubit and Bus. After properly normalizing the sideband amplitudes obtained from solving Eqn.~\ref{eq:matrixformBus}, it is straightforward to show that (see SI Note~\ref{sec:busmatrixtheory} for details) the normalized parametric qubit-Bus coupling of Q$_i$ is
\begin{equation}
    \label{eqn:gpar}
    \bar{g}_{i}=\frac{g_{\text{par},i}}{g_{0i}}=\frac{\frac{1}{2}(-1)^{i+1}\left(\tilde{\Phi}^{(1)}_{-}-\tilde{\Phi}^{(-1)}_{-}\right)}{\tilde{\phi}_{\text{in},0}(\omega_{\text{in},\text{r}})}\cos\left(\frac{\omega_{\text{f}}x_{i}}{v}\right)
\end{equation}
where the qubit position along the Bus is $x_{i}$ and the zero point phase field fluctuation of the initial unmodulated Bus mode is $\tilde{\phi}_{\text{in},0}(\omega_{\text{in},\text{r}})$. Thus, the parametric coupling rate is determined by the weights of the Bus sideband amplitudes in the presence of flux modulation.
%$g_{0i}=\frac{1}{2}\sqrt{\omega_{\text{q},i}\omega_{\text{r}}/\ell C_{0}C_{\text{q,i}}}C_{i,\text{r}}$ where $\omega_{\text{q},i}$ is the frequency of Q$_i$ with capacitance $C_{\text{q},i}$ and coupling capacitance $C_{i,\text{r}}$ between Q$_i$ and the Bus mode of interest.

In order to measure $g_{\text{par},i}$, we perform a three-tone frequency domain (FD) experiment with the Bus biased to $F=\pi/4$ (see Methods). As the phase correlated Bus flux modulation frequency $\omega_{\text{f}}$ is swept through the detuning $\Delta_{i}$ a parametric qubit-Bus avoided crossing is observed between the qubit and the first order Bus sidebands (see Fig.~\ref{fig:parametricqubitbus}\textbf{b}). The size of the avoided crossing is $2g_{\text{par},i}$. We repeat the measurement at multiple modulation amplitudes $\delta f$ and qubit-Bus detunings, $\Delta_{i}$ with the results shown in Fig.~\ref{fig:parametricqubitbus}\textbf{a} for a representative qubit, Q$_{4}$. Data for qubits Q$_{1}$, Q$_{6}$, Q$_{7}$, and Q$_{8}$ can be found in SI Note~\ref{sec:extdataFD}. The circuit parameters are constrained from the fit in Table~\ref{tab:DCfitpars} and $g_{0i}$ is similarly extracted from the avoided crossing observed by tuning Q$_i$ across the 8th order Bus mode. This leaves just a single free parameter in the model, the proportionality constant between the room temperature flux modulation amplitude in volts (V) and the corresponding modulation amplitude in units of $\pi$ after normalizing to the magnetic flux quantum $\Phi_{0}$. We find good agreement between the experimentally measured parametric coupling and the theoretical prediction for a microwave line attenuation of $31~\text{dB}$ which is in good agreement with the cryogenic line and room temperature cable attenuation estimated to be $30.3~\text{dB}$. We attribute the remaining difference to insertion loss in the bias tee used to combine the AC and DC flux biases.

The interaction occurs between the qubits and sidebands of the 8th order Bus mode which is designed to couple symmetrically to all qubits and has the frequency closest to the qubit frequencies. We verify that the qubits all interact symmetrically with the Bus by comparing their parametric couplings for the same modulation amplitude. In Fig.~\ref{fig:parametricqubitbus}\textbf{c} we see that the data all collapse onto a single curve. Based on Eqn.~\ref{eqn:gpar} this qubit position independent coupling is expected in the current case where $\omega_{\text{f}} \ll \omega_{\text{FSR}}$ and $\cos(\omega_{\text{f}}x_{i}/v) \approx 1$.

We corroborate these extensive frequency domain (FD) measurements with time domain (TD) measurements of the qubit-Bus coupling rate. These are performed by first exciting Q$_i$, then modulating the Bus boundary SQUIDs at $\omega_{\text{f}}=\Delta_{i}$ and observing coherent population exchange between the qubit and Bus (see Fig.~\ref{fig:parametricqubitbus}\textbf{e} for the pulse sequence). Repeating this for $\omega_{\text{f}}$ around $\Delta_{i}$ yields the characteristic TD chevron pattern from which the TD coupling rate is extracted from the population exchange rate. Fig.~\ref{fig:parametricqubitbus}\textbf{d} shows that the FD and TD measurements of the qubit-Bus coupling agree well after accounting for an extra $0.5~\text{dB}$ of attenuation from a DC block that was added to the Bus flux lines between the FD and TD measurements. The close agreement validates the frequency domain method for extracting the parametric coupling rates.

==> tunableresonator.tex <==
\begin{figure*}
    \centering
    \includegraphics{figure/circuitdiagramandchip_horizontal_fancy2.pdf}
    \caption{\textbf{a}, False colored, composite microscope image of the fabricated device. The device was fabricated through a flip-chip process with the qubit chip containing qubits and readout circuitry and the wiring chip containing control lines and the Bus (see Methods) \cite{Rosenberg20173D, Yost2020}. Qubits are labelled starting with Q$_{1}$ in the top left and wrapping around along the trace of the Bus (red) to Q$_{8}$ on the bottom left. \textbf{b}, Schematic showing two qubits coupled to the Bus resonator in the upper figure. In the lower figure, the Bus coupling mode wave profile seen by qubits for effective open-open boundaries (red), effective short-short boundaries (yellow), and effective open-short boundaries (green) as a function of position $x$ along the Bus. \textbf{c}, The measured Bus spectrum for the 7th mode as a function of flux bias at one boundary. The dots correspond to the bias points for profiles of the same colors in \textbf{b}. See Methods for measurement details. The multi-mode spectrum was used to extract Bus parameters through fitting to a double-side SQUID terminated CPW resonator model. \textbf{d}, Effective lumped LC circuit model for the Bus resonator constructed with a long coplanar waveguide terminated by SQUIDs at both ends. The magnetic flux through each SQUID, $f_{\pm}(t)$ is controlled by the Bus-Z flux line next to it.} 
    \label{fig:spidernetcircuit}
\end{figure*}

Linear coplanar waveguide (CPW) resonators are commonly used in superconducting quantum circuits to mediate coupling between transmon qubits \cite{ChowCR, Paik_RIPGate, Lu_MSGate}. The qubits are coupled capacitively to the CPW resonator in which case the qubit-resonator coupling, $\hbar g_{0i}=C_{i,\text{r}}V_{0,\mathrm{r}}(x_{i})V_{0,i}$ for qubit $i$, is determined by the zero point fluctuation voltage amplitude of the resonator mode profile $V_{0,\mathrm{r}}(x_{i})$ at the qubit position $x_{i}$, the qubit zero point voltage fluctuation $V_{0,i}=\sqrt{\frac{\hbar\omega_{\text{q},i}}{2C_{\text{q},i}}}$ for qubit frequency $\omega_{\text{q},i}$ and shunt capacitance $C_{\text{q},i}$, and capacitance between the qubit and resonator, $C_{i,\text{r}}$. The effective resonator mediated qubit-qubit coupling is approximately $g_{ij}=g_{i}g_{j}(1/\Delta_{i} + 1/\Delta_{j})$ where $\Delta_{i} =\omega_{\text{q},i}-\omega_{\text{r}}$ is the detuning between the frequencies of qubit $i$ and the resonator. Since $g_{ij} \sim V_{0,\mathrm{r}}(x_{i})V_{0,\mathrm{r}}(x_{j})$, if the field profile along the resonator can be tuned then the qubit-qubit coupling can also be tuned. 

For a CPW resonator, the mode profile will be determined by its geometry and boundary conditions. We use a resonator with tunable boundary conditions to mediate the qubit-qubit coupling \cite{CasparisVoltageTunableBus}. In this work, tunability is introduced by terminating the CPW resonator to ground through superconducting quantum interference devices (SQUIDs) \cite{Sandberg2008, Palacios-Laloy2008, Castellanos-Beltran2007} at both boundaries (see Fig.~\ref{fig:spidernetcircuit}\textbf{b}). The SQUIDs act like flux-tunable boundary impedances, $Z(\Phi)=\sqrt{L_{\mathrm{SQ}}(\Phi)/C_{\mathrm{SQ}}}$ where $L_{\mathrm{SQ}}(\Phi)=L_{\text{SQ}}(0)/\cos \Phi$ is the flux tunable Josephson inductance of the symmetric SQUID and $C_{\mathrm{SQ}}$ is the SQUID capacitance to ground. Let $Z_{0}$ be the impedance of the bulk CPW resonator, then proper design of the boundary SQUID allows for tuning the boundary condition from short, $Z(\Phi) \ll Z_{0}$, to open, $Z(\Phi) \gg Z_{0}$ \cite{JohanssonCasimir1,JohanssonCasimir2}. If the qubits are positioned at nodes (antinodes) of the mode profile with both boundary conditions tuned to open, then they will be positioned at antinodes (nodes) of the mode profile with both boundary conditions tuned to short, as depicted schematically in Fig.~\ref{fig:spidernetcircuit}\textbf{b}. As a result the qubit-resonator and qubit-qubit couplings can be tuned from nearly zero to a maximum value determined by flux-tunable circuit parameters. 

In an attempt to formalize the above intuition we now present an explicit circuit model of the tunable resonator. The circuit diagram is shown in Fig.~\ref{fig:spidernetcircuit}\textbf{d}. For concreteness, the length of the resonator is $\ell$ with the position along the resonator $-\ell/2 \leq x \leq \ell/2$. The capacitance and inductance per unit length in the bulk of the CPW are $C_{0}$ and $L_{0}$ respectively, giving a bulk CPW impedance of $Z_{0}=\sqrt{L_{0}/C_{0}}$. The junctions composing the boundary SQUIDs have capacitances $C_{si}$ and Josephson energies $E_{\mathrm{J},si}$ where $s=\pm$ denotes the $x= \pm \ell/2$ boundary and $i=1,2$ labels the junctions within each SQUID. The dynamical variables are the bulk node fluxes $\phi_{j}$ for $j=0,\dots,N$ and the boundary SQUID node fluxes $\phi_{s}$ for $s=\pm$. The time dependent external fluxes threading the boundary SQUIDs are $f_{s}(t)$. Our model for the system and subsequent calculations follow closely previous work in \cite{WustmannParametricResonance} and \cite{WallquistSelectiveCoupling} but are generalized to the case where both ends of the tunable resonator are terminated by SQUIDs to yield the equations of motion below. The details of this calculation can be found in SI Note~\ref{sec:busEOM}.

The bulk phase field, $\phi(x,t)$, satisfies
\begin{equation}
    \frac{\partial^{2}\phi}{\partial t^{2}}-v^{2}\frac{\partial^{2}\phi}{\partial x^{2}}=0
    \label{eqn:eombulk}
\end{equation}
which is simply the standard electromagnetic wave equation where $v=1/\sqrt{L_{0}C_{0}}$ is the speed of light in the bulk CPW. At the boundaries the phase field satisfies 
\begin{equation}
    \lim_{x \rightarrow \pm \frac{\ell}{2}}\left[\frac{2}{\omega_{\mathrm{J}}^{2}}\frac{\partial^{2}\phi}{\partial t^{2}}+2\cos f_{\pm}(t)\sin\phi \pm \eta d\frac{\partial \phi}{\partial x}\right]=0
    \label{eqn:eombndry}
\end{equation}
where $\omega_{\mathrm{J}}=\sqrt{2E_{\mathrm{C}}E_{\mathrm{J}}}/\hbar$ is the plasma frequency of the Josephson junctions composing the boundary SQUIDs, $E_{\mathrm{C}}=(2e)^{2}/2C_{\mathrm{J}}$ is the junction charging energy, and $\eta=E_{\mathrm{L}}/E_{\mathrm{J}}$ is the ratio of the bulk inductive energy $E_{\mathrm{L}}=\left(\frac{\Phi_{0}}{2\pi}\right)^{2}/\ell L_{0}$ to the boundary Josephson energy, $E_{\mathrm{J}}$. For simplicity we assume the SQUIDs are symmetric and that the SQUIDs at either boundary are identical. Thus the junction capacitance $C_{\mathrm{J}}=C_{si}$ and $E_{\mathrm{J}}=E_{\mathrm{J},si}$ for all $s$ and $i$. First we consider the case of DC flux bias $f_{\pm}(t)=F_{\pm}$. The resonant frequencies of the flux biased tunable resonator can be solved for numerically and fit to the experimentally measured tunable resonator mode spectrum in order to extract the circuit parameters, as outlined below.

We design and fabricate an eight-qubit version of the proposed architecture, shown in Fig.~\ref{fig:spidernetcircuit}\textbf{a}. The tunable resonator is a $10.55~\text{cm}$, chip-scale meander CPW resonator terminated by SQUIDs at either end. On-chip flux lines (Bus-Z) are used for DC and RF biasing of the boundary SQUIDs and a charge drive line (Bus-Drive) is used to spectroscopically probe the tunable resonator. Eight tunable transmon qubits are capacitively coupled to the Bus resonator. Each qubit has its own on-chip flux (Qubit-Z) and charge (Qubit-XY) control lines and a readout resonator. The eight readout resonators are all coupled to a single feed-line for multiplexed readout. 
%The state of the Bus resonator cannot be probed directly so its spectrum is measured by using a vector network analyzer (VNA) to monitor a weak probe tone at the frequency of one of the qubit readout resonators while sweeping a second tone sent to the Bus drive line. The chosen readout resonator's qubit acts as a spectrometer coupled to the Bus resonator. When the Bus is driven on resonance with one of its modes, the response of the spectrometer qubit is observed through its readout resonator. 

The measurement setup allows for observation of the first nine modes of the Bus which are spaced by the free spectral range (FSR) of $\omega_{\text{FSR}}\sim 2\pi \times 660~\text{MHz}$ up to approximately $2\pi \times 6~\text{GHz}$ (see Methods). The bus frequency is tuned by the boundary flux biases, $F_{\pm}$, which tune the boundary conditions. We fix $F_{+}=0$ and sweep $F_{-}$ over the range $-\pi/2 \leq F_{-} \leq \pi/2$ and measure the frequencies $\omega_{n,\text{r}}$ of Bus modes $n=1,\dots,9$ at each bias. Mode 7 and its fit to the theoretical model introduced above are shown in Fig.~\ref{fig:spidernetcircuit}\textbf{c} (extended data over the full frequency range is found in SI Note~\ref{sec:extdataFD}). Modes 3, 5, 6, 7, and 9 are simultaneously fit to a single set of circuit parameters. When the mode frequencies are normalized by the mode index, the fitted modes collapse onto each other while modes 1 and 8 are offset by $\mp 10~\text{MHz}$ so they are excluded from the fit. Modes 2 and 4 can be observed as well but they couple weakly to the qubit used as a spectrometer for these measurements so they are also excluded from the fit. Beyond observing strong agreement between the fit and experimental spectra, we also find that the fit circuit parameters are all within a reasonable range of their designed or simulated values, as given in Table~\ref{tab:DCfitpars}. To obtain a good fit, particularly near the $F_{-}=\pm \pi/2$ bias points, we need to allow for a small SQUID asymmetry, $d=(E_{\mathrm{J},1}-E_{\mathrm{J},2})/(E_{\mathrm{J},1}+E_{\mathrm{J},2})$ in the model. The fit value of $d=0.06$ is within a reasonable range for the typical fabrication variation in the junction critical currents. 
